RNR: Teaching Large Language Models to Follow Roles and Rules

Instruction fine-tuning (IFT) elicits instruction following capabilities and steers the behavior of large language models (LLMs) via supervised learning. However, existing models trained on open-source IFT datasets only have the ability to follow instructions from users, and often fail to follow complex role and rules specified by developers, a.k.a. system prompts. The ability to follow these roles and rules is essential for deployment, as it ensures that the model safely interacts with users within developer defined guidelines. To improve such role and rule following ability, we propose \model, an automated data generation pipeline that generates diverse roles and rules from existing IFT instructions, along with corresponding responses. This data can then be used to train models that follow complex system prompts. The models are evaluated on our newly created benchmarks for role and rule following ability, as well as standard instruction-following benchmarks and general NLP tasks. Our framework significantly improves role and rule following capability in LLMs, as evidenced by over 25% increase in pass-rate on rule adherence, i.e. following all requirements, in our experiments with the Alpaca and Ultrachat datasets. Moreover, our models achieves this increase without any regression on popular instruction following benchmarks.

==> tab_vicuna.tex <==

\begin{table*}[ht]
\caption{Pass rate on the main evaluation sets. Llama-2-7B is the base model for RNR.}
\label{tab:vicuna-benchmark}
\centering
\scalebox{0.8}{

\begin{tabular}{| c | c c |c c |c c | c c |}
\hline Closed LLM & \multicolumn{2}{| c |}{\textbf{In-house Eval} } & \multicolumn{2}{ c |}{\textbf{RolenruleEval} } & \multicolumn{2}{ c |}{\textbf{Alpacafarm-system} } & \multicolumn{2}{ c |}{\textbf{Average} }  \\ 
\cline{2-9}
 & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level  \\
\hline
Claude-2 & 94.22 & 88.0 & 83.05 & 65.15 & 93.71 & 85.48 & 90.33 & 79.54 \\
GPT4-Turbo & - & - & - & - & - & - & - & - \\
\hline 
\hline Open LLM & \multicolumn{2}{| c |}{\textbf{In-house Eval} } & \multicolumn{2}{ c |}{\textbf{RolenruleEval} } & \multicolumn{2}{ c |}{\textbf{Alpacafarm-system} } & \multicolumn{2}{ c |}{\textbf{Average} }  \\ 
\cline{2-9}
 & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level  \\
\hline
Vicuna-7b-v1.5 & 79.70 & 65.96 & 76.64 & 56.02 & 85.47 & 67.72 & 80.60 & 63.23 \\
Mistral-7B-Instruct-v0.1 & 86.96 & 70.0 & 76.51 & 55.39 & 88.10 & 73.33 & 83.86 & 66.24 \\
Zephyr-7b-beta & 70.58 & 64.44 & 79.15 & 54.98 & 91.46 & 78.83 & 80.40 & 66.08 \\
\hline 
\hline RNR:Alpaca & \multicolumn{2}{| c |}{\textbf{RNR-Expert} } & \multicolumn{2}{ c |}{\textbf{RNR-Awesome} } & \multicolumn{2}{ c |}{\textbf{RNR-Alpacafarm} } & \multicolumn{2}{ c |}{\textbf{Average} }  \\ 
\cline{2-9}
 & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level  \\
\hline


IFT: fixed-system & 53.62 & 39.53 & 58.39 & 28.6 & 72.57 & 43.21 & 61.53 & 37.11 \\
IFT: no-system & 64.76 & 57.78 & 67.59 & 39.05 & 74.41 & 44.47 & 68.92 & 47.10 \\
Rolenrule & \textbf{82.24} & \textbf{77.78} & \textbf{74.91} & \textbf{49.07} & \textbf{86.34} & \textbf{67.30} & \textbf{81.16} & \textbf{64.72} \\
\hline
\hline RNR:Ultrachat & \multicolumn{2}{| c |}{\textbf{In-house Eval} } & \multicolumn{2}{ c |}{\textbf{RolenruleEval} } & \multicolumn{2}{ c |}{\textbf{Alpacafarm-system} } & \multicolumn{2}{ c |}{\textbf{Average} } \\ 
\cline{2-9}
 & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level & Rule Level & Prompt Level  \\
\hline


IFT: fixed-system & 61.18 & 48.89 & 57.51 & 29.10 & 76.14 & 49.56 & 64.94 & 42.52 \\
IFT: no-system & 80.50 & 70.21 & 63.07 & 36.49 & 75.23 & 51.09 & 72.93 & 52.60  \\
Rolenrule & \textbf{85.56} & \textbf{75.0} & \textbf{75.17} & \textbf{49.59} & \textbf{89.56} & \textbf{74.37} & \textbf{83.43} & \textbf{66.32} \\
\hline
\end{tabular}}
\end{table*}


